DART: Domain-Adversarial Residual-Transfer Networks for Unsupervised Cross-Domain Image Classification

The accuracy of deep learning (e.g., convolutional neural networks) for an image classification task critically relies on the amount of labeled training data. Aiming to solve an image classification task on a new domain that lacks labeled data but gains access to cheaply available unlabeled data, unsupervised domain adaptation is a promising technique to boost the performance without incurring extra labeling cost, by assuming images from different domains share some invariant characteristics. In this paper, we propose a new unsupervised domain adaptation method named Domain-Adversarial Residual-Transfer (DART) learning of Deep Neural Networks to tackle cross-domain image classification tasks. In contrast to the existing unsupervised domain adaption approaches, the proposed DART not only learns domain-invariant features via adversarial training, but also achieves robust domain-adaptive classification via a residual-transfer strategy, all in an end-to-end training framework. We evaluate the performance of the proposed method for cross-domain image classification tasks on several well-known benchmark data sets, in which our method clearly outperforms the state-of-the-art approaches.

==> complementary.tex <==
\Section*{Supplementary materials}
We provide Algorithm description of DART in the supplementary material, followed by data description, and additional literature comparison.

\subsection{Algorithm Description}

To clearly express our DART model, we represent the pseudo-code in Algorithm.\ref{DART algorithm}.


% embedding them into domain classifier, and then we could minimize the loss function $L$ directly to attain optimal parameter $\theta_f$, $\theta_d$, $\theta_r$ instead of  maximizing  the loss function $L$ for optimal parameter $\theta_d$ and minimizing the loss function
%for $\theta_f$ and $\theta_r$. The GRL function $g$ has the same output as the identity function,  but reverses the gradient direction. Formally, for some function $f(v)$, the GRL function is defined as $g(f(v))=f(v)$ with a gradient $\frac{d}{dv}g(f(v))=-\frac{d}{dv}f(v)$. The equation of  $\hat{d}^s_i$ and $\hat{d}^t_i$ can be written as follow.




%\vspace{1.5ex}
%\hspace{-2.8ex}$\textbf{Remark:}$ The architecture of DJARTN is similar to RTN \cite{Long2016UnsupervisedDA}, but differs in the following ways: i) We learn domain-invariant features by reducing the joint distribution discrepancy instead of marginal distribution discrepancy, which could be robust since the marginal distributions are the subset of the joint distribution. ii) Instead of minimizing a MMD metric, we seek to adversarially train a domain classifier to reduce the domain discrepancy.




%The objective of this paper is to design a deep neural network
%that enables learning of adaptive classifier $y=f_s(x) $ and $y=f_t(x)$ to close the source-target discrepancy and reduce the joint discrepancy

\begin{algorithm}[t] 
\caption{\small The algorithm description for DART.}
%\textbf{Require:} 

%$x_i^s$, $y_i^s$ and $x_i^t$ representing source  samples, source  labels and target samples respectively.\\
%\textbf{Require:} domain classifier label $d_i^s =1$, $d_i^t =0$.\\
%\textbf{Require:}$\beta$,$\beta$, $\lambda(t)$ and $\eta(t)$  represent  regularizer for entropy penalty, domain classification, and ensembling regularization respectively.
%\textbf{Require:} random augmentation functions:$\hat{h}(\cdot)$, $\bar{h}(\cdot)$, $\tilde{h}(\cdot)$.\\
%\textbf{Require:} the student network $G_y(G_f(\cdot);\theta_y)$  with parameters $\theta_y$, the teacher network $G_y(G_f(\cdot);\hat{\theta}_y)$ represents  with parameters $\hat{\theta}_y$.\\
%\textbf{Require:} the domain classifier $G_d(\cdot)$ with parameters $\theta_d$.\\
%\textbf{Require:} the gradient reversal layer function $g(\cdot)$.

\begin{algorithmic}
\STATE Require:
\begin{itemize}
    \item source  samples and labels ($x_i^s,y_i^s$) and target samples $x_i^t$
    \item domain classifier label $d_i^s =1$, $d_i^t =0$
    \item trade-off parameter $\alpha$ and $\beta$ for entropy penalty and domain classification respectively
    and hyper-parameter $\lambda(t)$ for the gradient reversal layer function $g(\cdot;\lambda(t))$.
    \item the feature extractor $G_f(\cdot);\theta_f)$  with parameters $\theta_f$, 
    \item the domain classifier $G_d(\cdot)$ with parameters $\theta_d$
    \item the source classifier $G_s(\cdot;\theta_r)$
    with parameters $\theta_r$ and target classifier
    $G_t(\cdot)$
\end{itemize}
\FOR{$t$ in $[1,training\_steps]$ } 
  \FOR{minibatch $A,B$ } 
  \STATE Extract features from source samples and target samples:
  \STATE $f^s_i =G_f(x^s_{i\in{A}};\theta_f,t), f^t_i = G_f(x^t_{i\in{B}};\theta_f,t)$
  \STATE Obtain source label prediction and target label prediction:
  \STATE$\hat{y}^s_i = G_s(f^s_i;\theta_r,t), \hat{y}^t_i = G_t(f^t_i;t)$
  \STATE Fuse features and labels with a Kronecker product to represent joint representation:
  \STATE$z^s_i = f^s_i \otimes y^s_i, z^t_i = f^t_i \otimes \hat{y}^t_i$
  \STATE Embed joint representation into domain classifier:
  \STATE $d_i^s =  G_d(g(z^s_i;\lambda(t));\theta_d,t),\newline d_i^t = G_d(g(z^t_i;\lambda(t));\theta_d,t)$
  \STATE Update loss function of domain classifier:  
  \STATE $\mathcal{L}_D = -\frac{1}{|A|}\sum_{i\in A}d^s_i\log{\hat{d}^s_i}$
  \STATE $\qquad\:\:\:-\frac{1}{|B|}\sum_{i \in B}(1-d^t_i)\log{(1-\hat{d}^t_i)}$
  \STATE Update loss function of source classifier: \STATE$\mathcal{L}_Y =-\frac{1}{|A|}\sum_{i\in A}y_i^s \log{\hat{y}^s_i}$
  \STATE Update loss function of target classifier: \STATE$\mathcal{L}_H =-\frac{1}{|B|}\sum_{i\in B}\hat{y}^t_i \log{\hat{y}^t_i}$
  \STATE Update overall objective loss function: \STATE$\mathcal{L} = \mathcal{L}_Y+\alpha \mathcal{L}_H +\beta \mathcal{L}_D$
  \STATE  Update $\theta_f$,$\theta_d$ and $\theta_r$ using SGD optimizer
  \ENDFOR
\ENDFOR \newline
\textbf{Return} $\hat{\theta}_f,\theta_d,\theta_r$
\end{algorithmic}
\label{DART algorithm}
\end{algorithm}

\subsection{Datasets and Baselines}
$\textbf{\emph{USPS}}  \leftrightarrow  \textbf{\emph{MNIST}}:$ MNIST~\cite{lecun1998gradient}
contains 60000 training digit images and 10000 test digit images, and USPS~\cite{Denker1988NeuralNR} contains 7291 training images and 2007 test images. 
Images of both datasets are handwritten digits(0-9), apparent domain shifts can be observed as illustrated in Figure \ref{USPS and MNIST samples}.
For the transfer task from MNIST to USPS, we use the labeled MNIST dataset as the source domain and use unlabeled USPS dataset as the target domain, and vice versa for the transfer task from USPS to MNIST.



%\begin{figure}[htbp]
%\centering\includegraphics[width=3.35in]{USPS_MNIST.pdf}
%\caption{The first two rows represent examples from the USPS dataset, and the last two rows represent examples from the MNIST dataset}
%\label{USPS and MNIST samples}
%\end{figure}

%\begin{figure}[htbp]
%\centering\includegraphics[width=3.35in]{Amazon_Webcam.pdf}
%\caption{The first two rows represent examples from the \emph{Amazon} %dataset, and the last two rows represent examples from the %\emph{Webcam} dataset}
%\label{Amazon and Webcam  samples}
%\end{figure}

%\begin{figure}[htbp]
%\centering\includegraphics[width=3.3in]{Pascal_Imagenet.pdf}
%\caption{The first two rows represent examples from the \emph{Pascal} %dataset, and the last two rows represent examples from the %\emph{Imagenet} dataset}
%\label{Pascal and Imagenet samples}
%\end{figure}



\textbf{\emph{Office-31}}\footnote{http://office31.com.my}~\cite{Saenko2010AdaptingVC} is a standard benchmark for unsupervised domain adaptation. It consists of 4652 images and 31 common categories collected from three different domains: \emph{Amazon} (\textbf{A}) which contains 2817 images from amazon.com, \emph{DSLR} (\textbf{D}) which contains 498 images from digital SLR camera and \emph{Webcam} (\textbf{W}) which contains 795 images from the web camera.
Images drawn from \textbf{A} and \textbf{W} are shown in \ref{Amazon and Webcam  samples},  illustrating the domain shifts across different datasets.
We evaluate all methods on the following six transfer tasks: $\textbf{A} \to \textbf{W}$, $\textbf{D} \to \textbf{W}$, $\textbf{W} \to \textbf{D}$, $\textbf{A} \to \textbf{D}$, $\textbf{D} \to \textbf{A}$, $\textbf{W} \to \textbf{A}$, as done in~\cite{Long2017DeepTL,Long2016UnsupervisedDA}. 

\textbf{\emph{ImageCLEF-DA}}\footnote{http://imageclef.org/2014/adaptation} is a benchmark dataset for the \emph{ImageCLEF 2014} domain adaptation challenge, consisting of three public domains: \emph{Caltech-256}(\textbf{C}), \emph{ImageNet ILSVRC 2012}(\textbf{I}), and \emph{ Pascal VOC 2012}(\textbf{P}). Each domain contains 12 categories and  each category has 50 images. 
Similarly, the domain shifts can be easily observed from the example images of \textbf{P} and \textbf{I} shown in Figure \ref{Pascal and Imagenet  samples}.
We also consider all the possible six transfer tasks: $\textbf{I} \to \textbf{P}$, $\textbf{P} \to \textbf{I}$, $\textbf{I} \to \textbf{C}$, $\textbf{C} \to \textbf{I}$, $\textbf{C} \to \textbf{P}$, $\textbf{P} \to \textbf{C}$, as done in~\cite{Long2017DeepTL}. 


For MNIST to USPS and USPS to MNIST, we compare with three recent unsupervised domain adaptation algorithms: CoGAN~\cite{Liu2016CoupledGA}, pixelDA~\cite{Bousmalis2016UPD}, and UNIT~\cite{Liu2017UnsupervisedIT}.
CoGAN and UNIT seek to learn the indistinguishable features from the discriminator.
PixelDA is an effective method in unsupervised domain adaptation in which a generator is used to map data from the source domain to the target domain.
We choose these GANs-based baselines since it has been illustrated in~\cite{Goodfellow2014GenerativeAN} that GANs have more advantages over conventional kernel method (e.g., MMD) on reducing distribution discrepancy of domains.

%All these three methods are motivated by  GANs \cite{Goodfellow2014GenerativeAN} and they reduce the distribution discrepancy in an adversarial scheme. The state of the art GANs has demonstrated that adversarial way has more advantages over conventional kernel method (MMD) on reducing distribution discrepancy of domains.

For \emph{Office-31} and \emph{ImageCLEF-DA} datasets, in order to have a fair comparison with the latest algorithms in unsupervised domain adaptatoin, we choose the same baselines as reported in Joint Adaptation Network (JAN)~\cite{Long2017DeepTL}. Aside from JAN, other baselines include Transfer Component Analysis (TCA)~\cite{Pan2009DomainAV},
Geodesic Flow Kernel (GFK)~\cite{Gong2012GeodesicFK}, 
ResNet~\cite{He2016DeepRL},
Deep Domain Confusion (DDC)~\cite{Tzeng2014DeepDC}, 
Deep Adaptation Network (DAN)~\cite{Long2015LearningTF},
Residual Transfer Network (RTN)~\cite{Long2016UnsupervisedDA},
Domain-Adversarial Training of Neural Networks (DANN)~\cite{Ganin2015UnsupervisedDA}.
%todo: add GANs based models.

% TODO: chaode
%TCA is a transfer learning method based on the MMD-regularized
%Kernel PCA, while GFK is a manifold learning method that interpolates across infinite number of intermediate subspaces  to bridge domains. DDC is the first method that maximizes the domain-invariant features by regularizing the adaptation layer of the
%AlexNet using linear-kernel MMD. DAN embeds deep features of multiple layers into the reproducing kernel
%Hilbert spaces (RKHS) and reduces the discrepancy of different distributions using the multi-kernel MMD.
%DANN has been introduced in Section 1. RTN also considers learning the perturbation function by plugging several residual layers to the source classifier, and fuses the features of multiple layers with a Kronecker product to minimize their discrepancy via MMD. 
%JAN aligns the joint distributions of multiple domain-specific layers, and minimize the joint maximum mean discrepancy (JMMD) via the adversarial training.




\begin{figure}[h]
\centering
\subfigure[USPS and MNIST samples]{
\includegraphics[width=0.4\textwidth]{USPS_MNIST.pdf}
\label{USPS and MNIST samples}}
%\hspace{-0.2cm}
\subfigure[\emph{Amazon} and \emph{Webcam} samples]{\includegraphics[ width=0.4\textwidth]{Amazon_Webcam.pdf}\label{Amazon and Webcam  samples}}
%\hspace{-0.2cm}
\subfigure[\emph{Pascal} and \emph{Imagenet} samples]{\includegraphics[width=0.4\textwidth]{Pascal_Imagenet.pdf}\label{Pascal and Imagenet  samples}}
\caption{Experiment datasets: The first two rows in (a) (b) (c) represent examples from the USPS, \emph{Amazon} and \emph{Pascal} datasets, and the last two rows represent examples from the MNIST,\emph{Webcam} and  \emph{Imagenet} datasets
respectively.}
\vspace{-0.4cm}
\label{figMClass}
\end{figure}




%\input{./related_new.tex}
\subsection{Categories of Unsupervised Domain Adaptation Methods}

We show the categories of unsupervised domain adaptation methods in Table~\ref{uda:category}.

\begin{table*}[h]
	\centering
	\caption{Categories of Unsupervised Domain Adaptation Methods}
	\begin{tabular}{p{6cm}|p{5cm}|p{2cm}|p{2cm}}
    \hline Model & Discrepancy measure & Distribution assumption & Classifier Perturbation\\
    \hline
	  DDC~\cite{Tzeng2014DeepDC} & MMD & Marginal & no\\\hline
	  DAN~\cite{Long2015LearningTF}& MMD & Marginal &no\\\hline
	  DANN~\cite{ganin2016domain}& Domain Adversarial Loss & Marginal & no \\ \hline
      DSN~\cite{Bousmalis2016DomainSN} & MMD/Domain Adversarial Loss & Marginal & no \\\hline
      UNIT~\cite{Liu2017UnsupervisedIT} & GAN & Marginal & no \\\hline
      CoGAN~\cite{Liu2016CoupledGA} & GAN & Marginal & no \\\hline
      DTN~\cite{Taigman2016UnsupervisedCI} & GAN & Marginal & no \\\hline pixelDA~\cite{Bousmalis2016UPD} & GAN & Marginal & no \\\hline
      RTN~\cite{Long2016UnsupervisedDA}  & MMD & Marginal & yes \\\hline
      JDA~\cite{Long2013TransferFL} & MMD & Joint & no \\\hline
      JAN~\cite{Long2017DeepTL} & JMMD & Joint & no \\\hline
      DART(proposed) & Domain Adversarial Loss & Joint & yes \\\hline
	\end{tabular}
	\label{uda:category}
\end{table*}

\input{./related_new.tex}

==> introduction_old.tex <==
\section{Introduction}

In the recent years, deep neural networks have remarkably improved the state of the art performance for various machine learning problems and applications. These impressive gains have been partially attributed to the supervised learning on large-scale datasets~\cite{Lin2014MicrosoftCC,Russakovsky2015ImageNetLS} where massive amounts of labeled data are available. However, for those datasets whose labels are missing, manual labeling of oceans of training data is an expensive task to accomplish. 
%However, labeling and annotating a large dataset is an expensive task to accomplish.
To overcome this problem, there is a strong motivation to seek an alternative algorithm, which can leverage the labeled data from a related source domain to help classify the unlabeled data in the target domain. Unfortunately, a primary obstacle arises from the shift of data distributions across different domains, and it brings us to the unsupervised domain adaptation. 

%such algorithms suffers from the distribution shift across different domains, which poses a primary obstacle in adapting predictive models for the target task. This brings us to the unsupervised domain adaptation. 

Unsupervised domain adaptation~\cite{Pan2010ASO} is a classical method in machine learning that aims at tackling the domain shifts across two different domains.
%is machine learning in the presence of the shift between training and test distributions. 
One of the main approaches to unsupervised domain adaptation seeks to link the source and target domain via learning the domain-invariant feature representations, and train an adaptive classifier with knowledge from the source domain to make classifications in the target domain. 
Previous work focus on learning deep features via deep neural networks~\cite{long2015learning} by minimizing a distance metric of domain discrepancy, such as  Maximum Mean Discrepancy (MMD)~\cite{Gretton2006AKM}.
%and one of the popular domain discrepancy was measured by Maximum Mean Discrepancy (MMD)\cite{Gretton2006AKM}.
More recent success comes from the Generative Adversarial Networks (GANs)~\cite{Goodfellow2014GenerativeAN}, which verifies that an adversarial learning scheme could have more advantages over traditional ways in minimizing a distance metric of domain discrepancy. 
Inspired by GANs, a number of recent work based on adversarial learning are proposed~\cite{Tzeng2017AdversarialDD,Ganin2015UnsupervisedDA,Liu2016CoupledGA,Liu2017UnsupervisedIT,Taigman2016UnsupervisedCI,Bousmalis2016DomainSN,Bousmalis2016UnsupervisedPD,ganin2016domain}, and produce breakthrough results on the benchmark datasets.

%can learn more transferable features for domain adaptation  
%of domain adaptation.

Among the GANs-inspired models, DANN~\cite{ganin2016domain} is a noteworthy model. Based on the common low-dimensional features extracted by the feature extractor, DANN proposes a novel domain classifier borrowing the ideas from GANs. The domain classifier and feature extractor are trained adversarially, where the former seeks to discriminate the domain of features correctly, and the latter tries to learn indistinguishable features from source and target domains. Then a label classifier is deployed to classify the labels of the source domain and the target domain with the learned domain-invariant features.
%Among the GANs-inspired models, DANN \cite{ganin2016domain} is a noteworthy model. DANN maps data in the source domain and target domain into a common low-dimensional feature space via a weight-sharing feature extractor, and proposes a novel domain classifier, label the feature extracting from source domain one otherwise zero, and then embed the feature into the domain classifier to predict the label of feature. 
%In the training process, it minimizes the cross-entropy for the parameter of domain classifier to discriminate the label of feature correctly; on the other hand,
%it maximize the cross-entropy for the parameter of feature extractor to make features extracting from source and target domains indistinguishable.
Despite the success of DANN, it still suffers from two problems. First, it assumes that the source label classifier can be directly applied to the target domain, however, in practice there could be some small shifts across the label classifiers. %, as illustrated in \ref{source classifier and target classifier}.
Second, the label information in the source domain is not considered in learning the domain-invariant features. In other words, minimizing the discrepancy of marginal distributions (i.e., without label information) may have restrictive representation.

%may not perform as well as minimizing that of joint distributions (i.e., with label information) for the source domain and target domain, since the marginal distributions are the subset of the joint distributions.

%Although such adversarial training method is effective in extracting domain-invariant feature representations, DANN is problematic for the assumption that the source classifier trained with only source domain labeled data can be directly transferred to the target domain upon the learned domain-invariant feature representations is rather strong in practical applications. On the other hand, compared with reducing the joint distributions discrepancy, reducing the marginal distributions discrepancy is not best choice since the marginal distributions are the subset of the joint distribution.
–
\begin{figure}[htbp]
\centering\includegraphics[width=3.10in]{draw.pdf}
\caption{A well-trained source classifier may fail to label the data in target domain effectively. By adding a perturbation function, the target classifier performs better than the source classifier. Here the red dots and green triangles denote samples from the target domain. }

\label{source classifier and target classifier}
\end{figure}

To address these problems, we propose a novel domain adaptation model named as Deep Joint Adversarial Residual Transfer Network (DJARTN). In detail, the proposed architecture consists of three parts: the feature extractor, the label classifier, and the domain classifier.
%Inheriting a similar network architecture from DANN, DJARTN enjoys two more modifications. 
First, in order to model the  perturbation function across the label classifiers, we  insert the ResNet~\cite{He2016DeepRL} into the source label classifier, since ResNet has superior advantages in modelling the  perturbation via a shortcut connection, as verified in RTN~\cite{Long2016UnsupervisedDA}. With the learned perturbation function, the label classifier could be more robust and accurate, and an intuitive illustration is shown in
Figure \ref{source classifier and target classifier}.

%and this method is verified to perform better on the target domains, For example, the source classifier cannot classify target examples correctly as in Figure \ref{source classifier and target classifier}. 
%Note that most of the methods supposed that source classifier differ from the target classifier in general require at least a small set of labeled target examples per class, hence they can only be applied in the semi-supervised domain adaptation scenario\cite{Joachims1999TransductiveIF,Duan2009DomainTS,Yang2007CrossdomainVC}. However, we enable this classifier adaptation by inserting several layer into source classifier via ResNet\cite{He2016DeepRL}, similar approach has also been adapted in RTN\cite{Long2016UnsupervisedDA}.

Furthermore, our model is established under a more general assumption that the joint distribution of both data and labels in the source domain and the target domain are different, and seek to reduce their joint discrepancy. Since the labels in the target domain are unavailable, they are replaced by the predicted labels. Minimizing the joint discrepancy could produces better domain-invariant features than minimizing the marginal discrepancy, since the marginal distributions are the subset of the joint distributions.

%with the domain classifier and the feature extractor trained in an adversarial way.
%assume that the joint distribution of label and data are different in source and target domain instead of the marginal distributions, i.e., $p(\xt,\yt) \neq p(\xs,\ys)$. the advantage of this assumption is more general since the marginal distributions are the subset of the joint distribution.
%However, it is hard to obtain  the joint distribution of the features and labels precisely. To represent the joint distribution approximatively, we fuse the  features and labels with kronecker product.
%Finally, we reduce the joint distribution discrepancy by  embedding these joint representations to the domain classifier.

To evaluate the proposed model, extensive experiments on several benchmarks are conducted. We show that DART can outperform most state of the art methods over multiple tasks, indicating the superiority of both effectiveness and robustness of our model.

To summary, our contributions are two-folds:
\vspace{-2ex}
\begin{enumerate}
    \item Our work is the first to consider learning the perturbation function across label classifiers in the adversarial transfer network. \vspace{-2ex}
    \item Our work is the first to minimize the discrepancy of the joint distribution of both data and labels in the adversarial scheme.\vspace{-2ex}
\end{enumerate}

The rest of the paper is organized as follows. In section 2 we introduce the model. Section 3 discusses the experiment, followed by the related work in Section 4. In the end, we draw the conclusion and discuss some extensions of our model.

%empirical evidence suggests that the DJARTN approach outperforms several state of art methods on standard domain adaptation benchmarks.


==> related.tex <==
\section{Related work} \label{sec:related}
Unsupervised domain adaptation based on deep learning architectures can bridge different domains or tasks and mitigate the burden of manual labeling. The goal of domain adaptation is to reduce the domain discrepancy measured in various probability distributions of different domains. 
According to the distributions utilized in measuring the domain discrepancy, most previous work on domain adaptation with deep learning can be summarized into three categories: 
(1) methods with the assumption that the same conditional distribution is shared between the target domain and the source domain, i.e.,  $p(\yt| \xt)=p(\ys|\xs)$, 
and similar marginal distributions of features could be found in two domains, i.e,  $p(G_s(\xt)) \approx p(G_t(\xs))$, where $G_s(\cdot)$ and $G_t(\cdot)$ denote feature transformation functions and can be different.
%, or map data in source domain into target domain to ensure $p(G(\xs)) \approx p(\xt)$, where $G(\cdot)$ is the mapping function.  
(2) methods with the assumption that a perturbation exists between the conditional distribution ,i.e,  $p(\yt|\xt)=p(\ys|\xs) + \epsilon $, where $\epsilon$ is some perturbation noise, yet marginal distributions of features is similar (i.e., $p(G_s(\xt)) \approx p(G_t(\xs))$).
(3) methods with the assumption that not only the same conditional distribution is shared between the target domain and the source domain (i.e., $p(\yt| \xt)=p(\ys|\xs)$), but also similar joint distributions of extracted features and labels can be observed, i.e,  $p(G_s(\xt),\yt) \approx p(G_t(\xs),\ys)$.

%Most existing methods to address domain adaption is to learn domain-invariant feature representations. Beyond these methods, other approaches based on different assumptions to address unsupervised domain adaptation are available. Overall, most previous work can be summarized into three categories according to the assumptions on the probability distributions: (1) $p(\xt) \neq p(\xs)$ and $p(\yt| \xt)=p(\ys|\xs) $; (2) $p(\xt) \neq p(\xs)$ and  $p(\yt|\xt)=p(\ys|\xs)+ \epsilon $; (3) $p(\xt,\yt) \neq p(\xs,\ys)$ and $p(\yt| \xt)=p(\ys|\xs)$;

The most popular approaches in the first category are to learn domain-invariant features via deep neural networks or to map data in one domain to another.
%The most popular approaches based on the first assumption is to learn domain-invariant features via  deep neural networks and reduce its discrepancy or to generate data with the style of the source domain and the content of the target domain by feeding target domain data into a generator in GANs and then import these generated data into the source classifier. 
For example, DDC~\cite{Tzeng2014DeepDC} adopts a weight-shared neural architecture to extract features (i.e., $G_s(\cdot) = G_t(\cdot)$), and minimizes its discrepancy via MMD~\cite{Gretton2006AKM}, such that a representation that is both semantically meaningful and domain-invariant can be learned. Instead of reducing the discrepancy with a single layer, DAN~\cite{Long2015LearningTF} imposes restrictions on the discrepancy of several corresponding layers to learn more transferable feature via  MMD. Another work named as DANN~\cite{ganin2016domain} introduces a domain classifier borrowing the idea from
GANs~\cite{Goodfellow2014GenerativeAN} to help learn transferable features in an adversarial way.
%propose a domain classifier to classify features a to obtain domain-invariant features and its proposed domain cross-entropy is a  minimax loss, similar to GANs~\cite{Goodfellow2014GenerativeAN}.
%DANN~\cite{ganin2016domain} integrates a gradient reversal layer into the standard architecture to avoid maximize the domain cross-entropy in its feature extractor and minimize the domain cross-entropy in its domain classifier simultaneously to obtain domain-invariant features and its proposed domain cross-entropy is a  minimax loss, which is similar to GANs~\cite{Goodfellow2014GenerativeAN}.
DSN~\cite{Bousmalis2016DomainSN} introduces a private subspace for each domain which captures domain-specific properties and a shared subspace which captures common features between domains via  autoencoders.
UNIT~\cite{Liu2017UnsupervisedIT} and CoGAN~\cite{Liu2016CoupledGA} adopt GANs in their architecture to extract  indistinguishable features from discriminator. % from adversarial discriminators which we can not distinguish between domains.
DTN~\cite{Taigman2016UnsupervisedCI} and pixelDA~\cite{Bousmalis2016UPD} map data in the source domain to the target domain by a generator (i.e., $G_t(\cdot) $is an identity function).

Different from the first category of approaches, the second category relaxes the rather strong assumption that the source classifier can be applied directly to the target domain. Instead, it considers a more general scenario in practical applications and assumes that the source classifier and the target classifier differ
by a small perturbation function.
For instance, the perturbation function between the source classifier and the target classifier can be obtained from a small set of labeled target examples per class in the scenario of the semi-supervised domain adaption~\cite{Yang2007CrossdomainVC,Duan2009DomainTS}.
When handling the unsupervised domain adaptation problems, RTN~\cite{Long2016UnsupervisedDA} learns an adaptive classifier by adding residual modules into the source label classifier, fusing the features from multiple layers with a Kronecker product, and then minimizing its discrepancy via the MMD measure. 

The third category of approaches addresses the joint distribution adaptation by minimizing the joint distribution discrepancy. 
%Compared to the methods~\cite{Tzeng2015SimultaneousDT,Tzeng2014DeepDC,Ganin2015UnsupervisedDA,long2015learning} which mainly correct the shifts in the marginal distributions, 
This class of approaches takes the joint distribution of labels and features into account and is thus more general. A representative work is JDA~\cite{Long2013TransferFL}, which addresses the scenario where the source domain and the target domain are different in both marginal and joint distributions, and integrates both distributions with Principal Component Analysis (PCA) to construct feature
representations. JAN~\cite{Long2017DeepTL} addresses the same scenario via deep neural networks, and minimizes the joint distribution discrepancy via the JMMD measure.

Our proposed method integrates the advantages of both the second and the third category of approaches. In detail, it assumes that the source classifier and the target classifier differ
by a small perturbation function, i.e., $p(\yt|\xt)=p(\ys|\xs) + \epsilon$, and also assumes a joint distribution adaptation lies between the source domain and the target domain, i.e., $p(G_s(\xt),\yt) \approx p(G_t(\xs),\ys)$, $G_s(\cdot) = G_t(\cdot)$. Thus the proposed method can be expected to extract good quality domain-invariant features. This has also been verified in the experiment section.



%[Discussion with UNIT and other models]

